Language Models can Infer Action Semantics for Symbolic Planners from Environment Feedback

Symbolic planners can discover a sequence of actions from initial to goal states given expert-defined, domain-specific logical action semantics. Large Language Models (LLMs) can directly generate such sequences, but limitations in reasoning and state-tracking often result in plans that are insufficient or unexecutable. We propose Predicting Semantics of Actions with Language Models (PSALM), which automatically learns action semantics by leveraging the strengths of both symbolic planners and LLMs. PSALM repeatedly proposes and executes plans, using the LLM to partially generate plans and to infer domain-specific action semantics based on execution outcomes. PSALM maintains a belief over possible action semantics that is iteratively updated until a goal state is reached. Experiments on 7 environments show that when learning just from one goal, PSALM boosts plan success rate from 36.4% (on Claude-3.5) to 100%, and explores the environment more efficiently than prior work to infer ground truth domain action semantics.

==> tables/cand_trajs.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llrrrrrr}
    Sampling Methods & Candidate Trajs & \multicolumn{2}{c}{CNF Prediction Methods} \\
     & & \multicolumn{2}{c}{LLM+Rule-based} \\
     \cmidrule(lr){3-4}
     & & steps & acc \\
    \toprule
    \multirow{3}{*}{LLM} & 0 & 495 & 100 \\
    & 1 & 366 & 100 \\
    & 3 & 369 & 100 \\
    \midrule
    \multirow{3}{*}{LLM w/ prospect.} & 0 & 398 & 100 \\
    & 1 & 389 & 100 \\
    & 3 & 355 & 100 \\
    \bottomrule
\end{tabular}
\caption{\textit{Domain: \textsc{Termes}}. \color{blue} Key findings: more candidate trajs help LLM w/ prospect, but one candidate traj is enough for pure LLM prediction.}
\label{tab:cand_trajs}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{llrrrrrr}
%     Sampling Methods & Candidate Trajs & \multicolumn{6}{c}{CNF Prediction Methods} \\
%      & & \multicolumn{2}{c}{Rule-based} & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{LLM+Rule-based} \\
%      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%      & & steps & acc & steps & acc & steps & acc \\
%     \toprule
%     \multirow{3}{*}{LLM} & 0 & & & & & 495 & 100 \\
%     & 1 & & & & & 366 & 100 \\
%     & 5 & & & & & 369 & 100 \\
%     \midrule
%     \multirow{3}{*}{LLM w/ prospect.} & 0 & & & & & 398 & 100 \\
%     & 1 & & & & & 389 & 100 \\
%     & 5 & & & & & 355 & 100 \\
%     \bottomrule
% \end{tabular}
% \caption{\textit{Domain: \textsc{Termes}}.}
% \label{tab:cand_trajs}
% \end{table}

==> tables/failed_trajs.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llrrrrrr}
    Sampling Methods & Failed Trajs & \multicolumn{2}{c}{CNF Prediction Methods} \\
     & & \multicolumn{2}{c}{LLM+Rule-based} \\
     \cmidrule(lr){3-4}
     & & steps & acc \\
    \toprule
    \multirow{3}{*}{LLM} & 0 & 423 & 100 \\
    & 1 & 445 & 100 \\
    & 5 & 366 & 100 \\
    \midrule
    \multirow{3}{*}{LLM w/ prospect.} & 0 & 420 & 100 \\
    & 1 & 451 & 100 \\
    & 5 & 389 & 100 \\
    \bottomrule
\end{tabular}
\caption{\textit{Domain: \textsc{Termes}}. \color{blue} Key findings: more failed trajs help LLM action semantic prediction, but only one failed traj might be harmful (overfit).}
\label{tab:failed_trajs}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{llrrrrrr}
%     Sampling Methods & Failed Trajs & \multicolumn{6}{c}{CNF Prediction Methods} \\
%      & & \multicolumn{2}{c}{Rule-based} & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{LLM+Rule-based} \\
%      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%      & & steps & acc & steps & acc & steps & acc \\
%     \toprule
%     \multirow{3}{*}{LLM} & 0 & & & & & 423 & 100 \\
%     & 1 & & & & & 445 & 100 \\
%     & 3 & & & & & 366 & 100 \\
%     \midrule
%     \multirow{3}{*}{LLM w/ prospect.} & 0 & & & & & 420 & 100 \\
%     & 1 & & & & & 451 & 100 \\
%     & 3 & & & & & 389 & 100 \\
%     \bottomrule
% \end{tabular}
% \caption{\textit{Domain: \textsc{Termes}}.}
% \label{tab:failed_trajs}
% \end{table}

==> tables/llm_prior.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llrrrrrr}
    \toprule
    Sampling Methods & ASP methods & \multicolumn{6}{c}{\termes} \\
     \cmidrule(lr){3-8}
     & & NR & NR w/o & NES & NES w/o & Acc & Acc w/o \\
    \midrule
    Random & Rule-based & 69 & 1000 & 707 & 1013 & 100 & 76.6 \\
    Random w/ prospect. & Rule-based & 29 & 37 & 587 & 915 & 100 & 100 \\
    (\ourmethodshort) LLM & LLM+Rule-based & 21 & 26 & 408 & 389 & 100 & 100 \\
    \bottomrule
\end{tabular}
\caption{\textit{Domain: \textsc{Termes}}. Include absolute and delta}
\label{tab:llm_prior}
\end{table}

==> tables/main_results.tex <==
\begin{table}[ht]
% \setlength{\aboverulesep}{1pt}
% \setlength{\belowrulesep}{1pt}
\centering
% \small
% \tabcolsep 2pt
\begin{tabular}{lrrrrrrrrr}
    Sampling Methods & \multicolumn{9}{c}{CNF Prediction Methods} \\
     & \multicolumn{3}{c}{Rule-based} & \multicolumn{3}{c}{LLM} & \multicolumn{3}{c}{LLM+Rule-based} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
     & resets & steps & acc & resets & steps & acc & resets & steps & acc \\
    \toprule
    \textit{Domain: \textsc{Barman}} \\
    \quad Random \\
    \quad Random w/ prospect. \\
    \quad LLM \\
    \quad LLM w/ prospect. \\
    \toprule
    \textit{Domain: \textsc{Termes}} \\
    \quad Random \\
    \quad Random w/ prospect. \\
    \quad LLM \\
    \quad LLM w/ prospect. \\
    \toprule
    \textit{Domain: \textsc{Grippers}} \\
    \quad Random \\
    \quad Random w/ prospect. \\
    \quad LLM \\
    \quad LLM w/ prospect. \\
    % & \cmark & & & \cmark & & & & & & \color{gray} 3952 \\
    % & \cmark & \cmark & & \cmark & & & & & & 1742 \\
    % \cmark & & & & \cmark & & & & & & 305 \\
    % \cmark & & \cmark & & \cmark & & & & & & 269 \\
    % & \cmark & & \cmark & & & & & & & \color{gray} 705 \\
    % & \cmark & \cmark & \cmark & & & & & & & 1693  \\
    % \cmark & & & \cmark & & & & & & & \color{gray} 489 \\
    % \cmark & & \cmark & \cmark & & & & & & & 868 \\
    %     & \cmark & & \cmark & \cmark & & & & & & 752 \\
    % & \cmark & \cmark & \cmark & \cmark & & & & & & 296 \\
    % \cmark & & & \cmark & \cmark & & & & & & 166 \\
    % \cmark & & \cmark & \cmark & \cmark & & & & & & \bf 149 \\
    \bottomrule        
\end{tabular}
\caption{Our method vs. baselines.}
\label{tab:main_results}
\end{table}

==> tables/main_results_v0.tex <==
\begin{table}[ht]
% \setlength{\aboverulesep}{1pt}
% \setlength{\belowrulesep}{1pt}
\centering
\small
\tabcolsep 2pt
\begin{tabular}{cccccrrrrrrr}
    \multicolumn{3}{c}{Sampling Methods} & \multicolumn{2}{c}{CNF Prediction} & \multicolumn{7}{c}{Benchmarks (\# of executed steps)} \\
    LLM & Rand & SC & LLM & Rule-Based & barman & blocksworld & floortile & grippers & storage & termes & tyreworld \\
    \toprule
    & \cmark & & & \cmark & & & & & & \color{gray} 3952 \\
    & \cmark & \cmark & & \cmark & & & & & & 1742 \\
    \cmark & & & & \cmark & & & & & & 305 \\
    \cmark & & \cmark & & \cmark & & & & & & 269 \\
    & \cmark & & \cmark & & & & & & & \color{gray} 705 \\
    & \cmark & \cmark & \cmark & & & & & & & 1693  \\
    \cmark & & & \cmark & & & & & & & \color{gray} 489 \\
    \cmark & & \cmark & \cmark & & & & & & & 868 \\
        & \cmark & & \cmark & \cmark & & & & & & 752 \\
    & \cmark & \cmark & \cmark & \cmark & & & & & & 296 \\
    \cmark & & & \cmark & \cmark & & & & & & 166 \\
    \cmark & & \cmark & \cmark & \cmark & & & & & & \bf 149 \\
    \bottomrule        
\end{tabular}
\caption{Our method vs. baselines.}
\label{tab:main_results}
\end{table}

==> tables/no_error_msg.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrrr}
    \toprule
    Sampling Methods & \multicolumn{3}{c}{\termes} & \multicolumn{3}{c}{\grippers} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & NR & NES & Acc & NR & NES & Acc \\
    \midrule
    LLM & 100 & 384 & 76.6 & 91 & 410 & 100 \\
    LLM w/ prospect. & 100 & 1013 & 80.9 & 34 & 145 & 100 \\
    \bottomrule
\end{tabular}
\caption{Learning without error message}
\label{tab:no_err_msg}
\end{table}

==> tables/prospection_steps.tex <==
\begin{table}[ht]
% \setlength{\aboverulesep}{1pt}
% \setlength{\belowrulesep}{1pt}
\centering
% \small
% \tabcolsep 2pt
\begin{tabular}{llrrrrrr}
    Sampling Methods & Prospect. Steps & \multicolumn{2}{c}{CNF Prediction Methods} \\
     & & \multicolumn{2}{c}{LLM+Rule-based} \\
     \cmidrule(lr){3-4}
     & & steps & acc \\
    \toprule
    \multirow{3}{*}{Random w/ prospect.} & 1 & 554 & 78.5 \\
    & 5 & 2054 & 78.5 \\
    & 10 & 614 & 100 \\
    \midrule
    \multirow{3}{*}{LLM w/ prospect.} & 1 & 387 & 100 \\
    & 5 & 369 & 100 \\
    & 10 & 389 & 100 \\
    \bottomrule
\end{tabular}
\caption{\textit{Domain: \textsc{Termes}}. \color{blue} Key findings: number of steps (actions) for prospection matters more when the trajectory sampler is random. Small number of prospection is enough for language model trajectory sampler.}
\label{tab:prospct_steps}
\end{table}

% \begin{table}[h]
% \centering
% % \small
% % \tabcolsep 2pt
% \begin{tabular}{llrrrrrr}
%     Sampling Methods & Prospect. Steps & \multicolumn{6}{c}{CNF Prediction Methods} \\
%      & & \multicolumn{2}{c}{Rule-based} & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{LLM+Rule-based} \\
%      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%      & & steps & acc & steps & acc & steps & acc \\
%     \toprule
%     \multirow{3}{*}{Random w/ prospect.} & 1 & & & & & 554 & 78.5 \\
%     & 5 & & & & & 2054 & 78.5 \\
%     & 10 & & & & & 614 & 100 \\
%     \midrule
%     \multirow{3}{*}{LLM w/ prospect.} & 1 & & & & & 387 & 100 \\
%     & 5 & & & & & 369 & 100 \\
%     & 10 & & & & & 389 & 100 \\
%     \bottomrule
% \end{tabular}
% \caption{\textit{Domain: \textsc{Termes}}.}
% \label{tab:prospct_steps}
% \end{table}

==> tables/rand_baselines.tex <==
\begin{table}[ht]
\centering
\small
\caption{Pure random baseline and random w/ prospect. baseline on 7 domains.}
\begin{tabular}{lrrrrrrrrrrrrrrr}
    \toprule
    Methods & \multicolumn{3}{c}{\termes} & \multicolumn{3}{c}{\grippers} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & NR & NES & Acc & NR & NES & Acc \\
    \midrule
    Rand-TS+Rule-ASP & 100 & 384 & 76.6 & 91 & 410 & 100 \\
    Rand-TS+Rule-ASP w/ prospect. & 100 & 1013 & 80.9 & 34 & 145 & 100 \\
    \bottomrule
\end{tabular}
\label{tab:no_err_msg}
\end{table}

==> tables/var_llm.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llrrrrrr}
\toprule
    Sampling Methods & LLM & \multicolumn{3}{c}{\termes} \\
    \cmidrule(lr){3-5}
     & & NR & NES & Acc \\
    \midrule
    \multirow{3}{*}{LLM} & GPT-4 & 24 & 366 & 100 \\
    & GPT-3.5 & 31 & 440 & 100 \\
    % & LLaMa-2 7B \\
    & Mistral 7B & 38 & 472 & 100 \\
    \midrule
    \multirow{3}{*}{LLM w/ prospect.} & GPT-4 & 21 & 389 & 100 \\
    & GPT-3.5 & 24 & 409 & 100 \\
    % & LLaMa-2 7B \\
    & Mistral 7B & 26 & 421 & 100 \\
    \bottomrule
\end{tabular}
\caption{\textit{Domain: \textsc{Termes}}.}
\label{tab:var_llm}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{llrrrrrr}
%     Sampling Methods & LLM & \multicolumn{6}{c}{CNF Prediction Methods} \\
%      & & \multicolumn{2}{c}{Rule-based} & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{LLM+Rule-based} \\
%      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%      & & steps & acc & steps & acc & steps & acc \\
%     \toprule
%     \multirow{5}{*}{LLM} & GPT-4 \\
%     & GPT-3.5 \\
%     & Gemini \\
%     & LLaMa-3 \\
%     & Mistral \\
%     \midrule
%     \multirow{5}{*}{LLM w/ prospect.} & GPT-4 \\
%     & Claude 3 \\
%     & Gemini \\
%     & LLaMa-3 \\
%     & Mistral \\
%     \bottomrule
% \end{tabular}
% \caption{\textit{Domain: \textsc{Termes}}.}
% \label{tab:var_llm}
% \end{table}
